Dynamical Analysis of Blocking Events: Spatial and Temporal Fluctuations of Covariant Lyapunov Vectors

One of the most relevant weather regimes in the mid-latitudes atmosphere is the persistent deviation from the approximately zonally symmetric jet to the emergence of blocking patterns. Such configurations are usually connected to exceptional local stability properties of the flow which come along with an improved local forecast skills during the phenomenon. It is instead extremely hard to predict onset and decay of blockings. Covariant Lyapunov Vectors (CLVs) offer a suitable characterization of the linear stability of a chaotic flow, since they represent the full tangent linear dynamics by a covariant basis which explores linear perturbations at all time scales. Therefore, we assess whether CLVs feature a signature of the blockings. As a first step, we examine the CLVs for a quasi-geostrophic beta-plane 2-layer model in a periodic channel baroclinically driven by a meridional temperature gradient $\Delta T$. An orographic forcing enhances the emergence of localized blocked regimes. We detect the blocking events with a Tibaldi-Molteni scheme adapted to the periodic channel. When blocking occurs, the global growth rates of the fastest growing CLVs are significantly higher. Hence, against intuition, the circulation is globally more unstable in blocked phases. Such an increase in the finite time Lyapunov exponents with respect to the long term average is attributed to stronger barotropic and baroclinic conversion in the case of high temperature gradients, while for low values of \Delta T, the effect is only due to stronger barotropic instability. In order to determine the localization of the CLVs we compare the meridionally averaged variance of the CLVs during blocked and unblocked phases. We find that on average the variance of the CLVs is clustered around the center of blocking. These results show that the blocked flow affects all time scales and processes described by the CLVs.

==> hylatex.ltx <==
%
% hylatex.ltx
% Tanmoy Bhattacharya and Sebastian Rahtz, June 1995
%
% Use this file to make a format which includes the
% hyperref package in every LaTeX job.
%
% In web2c 7-based TeX world, we create the format file with
%   tex  -ini \&latex hylatex.ltx
% and then use with
%   tex \&hylatex
%
% In teTeX (TeX version 3.14159 (C version 6.1), LaTeX2e <1996/12/01>
% patch level 1), I create the format file with
%   initex \&latex hylatex.ltx
% and then use with
%   virtex \&hylatex
%
% This method is not supported by the LaTeX2e team, so
% I will try to find a better way. \AtBeginDocument does not
% work for reasons which I do not understand.
%
\makeatletter
\expandafter\everyjob\expandafter{\the\everyjob
 \typeout{ ********* Hyperref Macros loaded ******* }}
%
\expandafter\let\csname REAL document\endcsname\document
%
\def\document{%
 \endgroup
%
% NOTE:
% This setup sets up no options by default;
% change to suit your needs, by writing a hyperref.cfg control
% file.
%
 \RequirePackage{hyperref}
 \begingroup
 \@endpefalse\csname REAL document\endcsname
}
\makeatother
\dump


